Hybrid Data-Free Knowledge Distillation

Data-free knowledge distillation aims to learn a compact student network from a pre-trained large teacher network without using the original training data of the teacher network. Existing collection-based and generation-based methods train student networks by collecting massive real examples and generating synthetic examples, respectively. However, they inevitably become weak in practical scenarios due to the difficulties in gathering or emulating sufficient real-world data. To solve this problem, we propose a novel method called \textbf{H}ybr\textbf{i}d \textbf{D}ata-\textbf{F}ree \textbf{D}istillation (HiDFD), which leverages only a small amount of collected data as well as generates sufficient examples for training student networks. Our HiDFD comprises two primary modules, \textit{i.e.}, the teacher-guided generation and student distillation. The teacher-guided generation module guides a Generative Adversarial Network (GAN) by the teacher network to produce high-quality synthetic examples from very few real-world collected examples. Specifically, we design a feature integration mechanism to prevent the GAN from overfitting and facilitate the reliable representation learning from the teacher network. Meanwhile, we drive a category frequency smoothing technique via the teacher network to balance the generative training of each category. In the student distillation module, we explore a data inflation strategy to properly utilize a blend of real and synthetic data to train the student network via a classifier-sharing-based feature alignment technique. Intensive experiments across multiple benchmarks demonstrate that our HiDFD can achieve state-of-the-art performance using 120 times less collected data than existing methods. Code is available at https://github.com/tangjialiang97/HiDFD.

==> sec/6_sup.tex <==
\clearpage
\appendix
\renewcommand{\thefigure}{A-\arabic{figure}}
\renewcommand{\thetable}{A-\arabic{table}}
\renewcommand{\thealgorithm}{A-\arabic{algorithm}}
\setcounter{figure}{0}
\setcounter{table}{0}
\section{Proofs}
\label{sup_proof}
\subsection{The Optimal Classifier of Discriminator}
\label{sup_proof1}
For a fixed generator, the optimal classifier $\Psi_{\mathrm{D}}^*$ of the discriminator in our employed Auxiliary Discriminative Classifier GAN (ADCGAN) can be formatted as follows:
\begin{equation}
\Psi_{\mathrm{D}}^*\left(y^{+} \mid \boldsymbol{x}\right)=\frac{p(\boldsymbol{x}, y)}{p(\boldsymbol{x})+q(\boldsymbol{x})}, \quad  \Psi_{\mathrm{D}}^*\left(y^{-} \mid \boldsymbol{x}\right)=\frac{q(\boldsymbol{x}, y)}{p(\boldsymbol{x})+q(\boldsymbol{x})}.
\end{equation}
\begin{proof}
	\begin{equation}
	\max_{\Psi_{\mathrm{D}}}\mathbb{E}_{\boldsymbol{x},y\sim P_{X,Y}}[\log \Psi_{\mathrm{D}}(y^+|\boldsymbol{x})] + \mathbb{E}_{\boldsymbol{x},y\sim Q_{X,Y}}[\log \Psi_{\mathrm{D}}(y^-|\boldsymbol{x})]
	\Rightarrow\max_{\Psi_{\mathrm{D}}}\mathbb{E}_{\boldsymbol{x},y\sim P^m_{X,Y}}[\log \Psi_{\mathrm{D}}(y|\boldsymbol{x})],
	\end{equation}
	with $p^m(\boldsymbol{x},y^+)=\frac{1}{2}p(\boldsymbol{x},y)$, $p^m(\boldsymbol{x},y^-)=\frac{1}{2}q(\boldsymbol{x},y)$, and $p^m(\boldsymbol{x})=\sum_y p^m(\boldsymbol{x},y)=\frac{1}{2}p(\boldsymbol{x})+\frac{1}{2}q(\boldsymbol{x})$.
	\begin{IEEEeqnarray}{rCl}
	&\Rightarrow&\max_{\Psi_{\mathrm{D}}}\mathbb{E}_{\boldsymbol{x}\sim P^m_{X}}\mathbb{E}_{y\sim P^m_{Y|X}}[\log \Psi_{\mathrm{D}}(y|\boldsymbol{x})]\\&\Rightarrow&\min_{\Psi_{\mathrm{D}}}\mathbb{E}_{\boldsymbol{x}\sim P^m_{X}}\mathbb{E}_{y\sim P^m_{Y|X}}[-\log \Psi_{\mathrm{D}}(y|\boldsymbol{x})]\\
	&\Rightarrow&\min_{\Psi_{\mathrm{D}}} \mathbb{E}_{\boldsymbol{x}\sim P^m_X}[H(p^m(y|\boldsymbol{x}))+\mathrm{KL}(p^m(y|\boldsymbol{x})\|\Psi_{\mathrm{D}}(y|\boldsymbol{x}))] \\
	&\Rightarrow& \Psi_{\mathrm{D}}^*(y|\boldsymbol{x})=\arg\min_{\Psi_{\mathrm{D}}}\mathrm{KL}(p^m(y|\boldsymbol{x})\|\Psi_{\mathrm{D}}(y|\boldsymbol{x}))=p^m(y|\boldsymbol{x})=\frac{p^m(\boldsymbol{x},y)}{p^m(\boldsymbol{x})}
	\end{IEEEeqnarray}
	Therefore, the optimal discriminative classifier of ADC-GAN has the form of $\Psi_{\mathrm{D}}^*(y^+|\boldsymbol{x})=\frac{p^m(\boldsymbol{x},y^+)}{p^m(\boldsymbol{x})}=\frac{p(\boldsymbol{x},y)}{p(\boldsymbol{x})+q(\boldsymbol{x})}$ and $\Psi_{\mathrm{D}}^*(y^-|\boldsymbol{x})=\frac{p^m(\boldsymbol{x},y^-)}{p^m(\boldsymbol{x})}=\frac{q(\boldsymbol{x},y)}{p(\boldsymbol{x})+q(\boldsymbol{x})}$ that conclude the proof.
\end{proof}
\subsection{Proof of Eq.~\eqref{eq_gl}}
\label{sup_proof2}
Given the optimal classifier of the discriminator proofed in Section~\ref{sup_proof1}, at the equilibrium point, encouraging the generator to produce easily classifiable examples of our employed ADCGAN is equivalent to
\begin{equation}
\max_{\mathcal{N}_\mathrm{G}}[\mathbb{E}_{\boldsymbol{x}, y \sim Q_{X, Y}}[\log \Psi^{*}_{\mathrm{D}}(y^{+}\mid\boldsymbol{x})]\!-\!\mathbb{E}_{\boldsymbol{x}, y \sim Q_{X, Y}}[\log \Psi^{*}_{\mathrm{D}}(y^{-}\mid\!\boldsymbol{x})]]\Rightarrow\min _{\mathcal{N}_\mathrm{G}} \mathrm{KL}\left(Q_{X, Y} \| P_{X, Y}\right),
\end{equation}
\begin{proof}
	\begin{IEEEeqnarray}{rCl}
	&&\max_{\mathcal{N}_\mathrm{G}} \mathbb{E}_{\boldsymbol{x},y\sim Q_{X,Y}}\left[\log \Psi_{\mathrm{D}}^*(y^+|\boldsymbol{x})\right] - \mathbb{E}_{\boldsymbol{x},y\sim Q_{X,Y}}\left[\log \Psi_{\mathrm{D}}^*(y^-|\boldsymbol{x})\right]\\
	&\Rightarrow&\max_{\mathcal{N}_\mathrm{G}} \mathbb{E}_{\boldsymbol{x},y\sim Q_{X,Y}}\left[\log \frac{p(\boldsymbol{x},y)}{p(\boldsymbol{x})+q(\boldsymbol{x})}\right] - \mathbb{E}_{\boldsymbol{x},y\sim Q_{X,Y}}\left[\log \frac{q(\boldsymbol{x},y)}{p(\boldsymbol{x})+q(\boldsymbol{x})}\right] \\
	&\Rightarrow&\min_{\mathcal{N}_\mathrm{G}}\mathbb{E}_{\boldsymbol{x},y\sim Q_{X,Y}}\left[\log \frac{q(\boldsymbol{x},y)}{p(\boldsymbol{x},y)}\right]\Rightarrow \min_{\mathcal{N}_\mathrm{G}} \mathrm{KL}(Q_{X,Y}\|P_{X,Y})
	\end{IEEEeqnarray}
\end{proof}
\begin{table}[t]
	\centering
	\caption{Details of the benchmark datasets used in our experiment, the items with the prefix ``\#" denotes the number of the corresponding item.}
	\setlength{\tabcolsep}{1.5mm}
	{
		\begin{tabular}{cccccc}
			\hline
			Dataset   &Type   & Image size  &\#classes & \#train & \#test \\ \hline
			CIFAR10   &Original data   & 32$\times$32             & 10        & 50,000  & 10,000 \\ 
			CIFAR100  &Original data   & 32$\times$32              & 100       & 50,000  & 10,000 \\ 
			CINIC     &Original data   & 32$\times$32             & 10        & 90,000  & 90,000 \\ 
			TinyImageNet&Original data  & 64$\times$64              & 200       & 100,000 & 10,000 \\ 
			HAM &Original data & 224$\times$224              & 7       & 8,000 & 2,000 \\ 
			ISIC &Collected data & 224$\times$224              & 8       & 20,000 & 5,000 \\ 
			ImageNet &Original\&collected data & 224$\times$224              & 1,000       & 1,281,167 & 50,000 \\
			WebVision &Collected data & 224$\times$224              & 1,000       & 980,449 & N/A \\ \hline
	\end{tabular}}
	\label{table_dataset}
\end{table}
\begin{figure}[t]
	\centering
	\includegraphics[scale=0.43]{img/sup_isic.pdf}
	\caption{The number of examples per category in the collected data ($\rho=0.1$), where the original data is (a) CIFAR10 and (b) HAM, respectively.}
	\label{fig_isic}
\end{figure}
\begin{algorithm}[t]
	\caption{Hybrid Data-Free Distillation}
	\begin{algorithmic}[1]
		\REQUIRE Pre-trained teacher network $\mathcal{N}_{\mathrm{T}}$, limted collected data $\mathcal{D}_{\mathrm{c}}$.
		\STATE Initialize the discriminator $\mathcal{N}_{\mathrm{D}}$ and generator $\mathcal{N}_{\mathrm{G}}$ in GAN, and the small student network $\mathcal{N}_{\mathrm{S}}$;
		\STATE \textbf{Module 1: Generative Distillation}
		\REPEAT 
		\STATE Sample the noise-label pair $(\boldsymbol{z}, y)$ to generate synthetic example $\mathcal{N}_\mathrm{G}(\boldsymbol{z}, y)$;
		\STATE Mitigate the overfitting of discriminator $\mathcal{N}_{\mathrm{D}}$ via blending $\mathcal{L}_{\mathrm{blend}}$ and transferring $\mathcal{L}_{\mathrm{trans}}$ operations in feature integration;
		\STATE Calculate the class frequency $\{\hat{n}_{c}\}_{c=1}^{C}$ of synthetic examples;
		\STATE Regularize the training of generator $\mathcal{N}_{\mathrm{G}}$ across all categories;
		\STATE Optimize the GAN via Adam;
		\UNTIL {convergence}
		\STATE \textbf{Module 1: Student Distillation}
		\STATE Generate abundant high-quality synthetic examples and inflate collected examples to construct the hybrid data $\mathcal{D}$; 
		\REPEAT 
		\STATE Sample the example $\boldsymbol{x} \in \mathcal{D}$ and input it into the teacher network $\mathcal{N}_{\mathrm{T}}$ and student network $\mathcal{N}_{\mathrm{S}}$ to obtain the features $\Phi_{\mathrm{T}}(\boldsymbol{x})$ and $\Phi_{\mathrm{S}}(\boldsymbol{x})$, respectively.
		\STATE Align the features $\Phi_{\mathrm{T}}(\boldsymbol{x})$ and $\Phi_{\mathrm{S}}(\boldsymbol{x})$ via $\mathcal{L}_{\mathrm{align}}$;
		\STATE Optimize the student network $\mathcal{N}_{\mathrm{S}}$ via SGD;
		\UNTIL {convergence}
		\ENSURE Lightweight student network $\mathcal{N}_{\mathrm{S}}$.
	\end{algorithmic}
	\label{alg_1}
\end{algorithm}
\section{Detailed Information of Benchmark Datasets}
\label{sup_dataset}
\subsection{Comprehensive Dataset Overview}
In Table~\ref{table_dataset}, we introduce the critical information of the benchmark datasets used in our experiment, including the image size, the number of categories, and the number of images in training and test sets. First, we can observe that the large-scale ImageNet contains a large number of examples, when using it as the original data, it is difficult to collect sufficient examples (more than 1 million) from the real-world. Therefore, it is essential to explore an efficient data-free distillation method that requires only a small amount of collected data. Second, a series of benchmark datasets contain 224$\times$224 sized high-resolution images, the generation-based methods that without rely on real-world data are hard to generate high-quality examples to provide effective information for training the student network.

Moreover, Figure~\ref{fig_isic} shows the number of collected examples in each category when the original data is the natural image datasets CIFAR10 and practical medical image dataset HAM, respectively. We can observe that the collected examples exhibit imbalanced class distribution, with several categories accounting for the majority of examples and other categories containing only a few examples. Therefore, our proposed data-free distillation method is very practical.
\begin{figure}[t]
	\centering
	\includegraphics[scale=0.24]{img/sup_cifar10.png}
	\caption{Visualization of synthetic examples for the original tasks, including (a) CIFAR10, (b) CINIC, (c) TinyImageNet, and (d) HAM.}
	\label{fig_vis_cifar10}
\end{figure}
\subsection{Visualization of Synthetic Examples}
In Figure~\ref{fig_vis_cifar10}, we show synthetic examples produced by the GAN trained on limited collected data using our generative distillation module. Specifically, we generate synthetic instances for four original datasets, including CIFAR10, CINIC, TinyImageNet, and HAM. Despite these original datasets having significantly different image sizes (ranging from 32$\times$32 to 224$\times$224), the corresponding synthetic examples consistently exhibit high quality. These visual results demonstrate the effectiveness of our approach in leveraging the teacher network to address critical issues of GAN training on limited collected data. By doing so, our method can train reliable student networks on abundant high-quality synthetic examples.
\section{Algorithm}
\label{sup_alg}
The detailed training algorithm of our proposed HiDFD is summarized in Algorithm~\ref{alg_1}. Our HiDFD contains two primary modules to train a reliable student network only using a small number of collected examples, \textit{i.e.}, the generative distillation and student distillation. In the generative distillation, the GAN is trained on the limited collected data under the guidance of the teacher network, where the critical issues, \textit{i.e.}, overfitting of the discriminator and imbalanced learning of the generator, are effectively resolved. In the student network, the collected examples are properly inflated via repeating and combined with sufficient high-quality synthetic examples to construct the hybrid data. Then, the reliable student network can naturally train on the hybrid data via the effective classifier-sharing-based feature alignment strategy.
\section{Limitations and Broader Impacts}
\label{sup_impact}
\subsection{Limitations}
The proposed method can train reliable student networks using very few collected examples. Compared with previous methods, we have reduced the data requirement by 99\%, making our method suitable for practical applications. In general, the effectiveness of the proposed method depends on the quality and representativeness of collected data to some extent. If this collected data does not sufficiently represent the broader dataset or contains biases, the generated synthetic examples and the trained student network may inherit these flaws. In practice, collecting fewer representative examples in real-world applications is relatively easy. Therefore, we believe that these limitations can be overcome well.
\subsection{Broader Impacts}
This paper proposed a novel data-free knowledge distillation method called HiDFD, which can train a compact and reliable student network using very few collected examples. In general, the proposed HiDFD could have the following positive impacts: 1) HiDFD eliminates the need for original training data required by traditional knowledge distillation methods, so it can help preserve data privacy for users; 2) HiDFD effectively compresses the large pre-trained models (\textit{i.e.}, the teacher networks) into smaller and faster models (\textit{i.e.}, the student networks) that are resource-efficient and suitable for deployment on devices with limited capabilities; 3) HiDFD focuses on the classification tasks, which underpin many practical downstream tasks like object detection and segmentation, suggesting its wide applicability; and 4) HiDFD is compatible with different DNNs (\textit{e.g.}, ResNet and VGG). 

Although HiDFD has few negative social impacts, when it compresses the large models of many Artificial Intelligence (AI) technologies and enables these compressed models in practical applications, the proposed HiDFD can be used for good and also for harm, depending on human intent. This actually falls into the general ethical debate on whether AI is good or not. 

In conclusion, we believe our proposed work can be beneficial to society since many important real-world applications need compact and reliable models that stand to benefit from HiDFD when the available real-world data is limited.

==> sec/check_list.tex <==
\newcommand{\answerYes}[1]{\textcolor{blue}{#1}} 
\newcommand{\answerNo}[1]{\textcolor{teal}{#1}} 
\newcommand{\answerNA}[1]{\textcolor{gray}{#1}} 
\newcommand{\answerTODO}[1]{\textcolor{red}{#1}}





\section{Reproducibility Checklist}

\begin{enumerate}
	
	\item This paper:
	\begin{enumerate}
		\item  Includes a conceptual outline and/or pseudocode description of AI methods introduced
		\answerTODO{Yes}
		\item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results
		\answerTODO{Yes}
		\item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper
		\answerTODO{Yes}
	\end{enumerate}
	
	\item Does this paper make theoretical contributions? \answerTODO{Yes}
	\begin{enumerate}
		\item All assumptions and restrictions are stated clearly and formally.
		\answerTODO{Yes}
		\item  All novel claims are stated formally (\textit{e.g.}, in theorem statements).
		\answerTODO{Yes}
		\item Proofs of all novel claims are included.
		\answerTODO{Yes}
		\item Proof sketches or intuitions are given for complex and/or novel results. 
		\answerTODO{Yes}
		\item Appropriate citations to theoretical tools used are given.
		\answerTODO{Yes}
		\item All theoretical claims are demonstrated empirically to hold.
		\answerTODO{Yes}
		\item All experimental code used to eliminate or disprove claims is included.
		\answerTODO{Yes}
	\end{enumerate}
	
	\item Does this paper rely on one or more datasets? \answerTODO{Yes}
	\begin{enumerate}
		\item A motivation is given for why the experiments are conducted on the selected datasets.
		\answerTODO{Yes}
		\item All novel datasets introduced in this paper are included in a data appendix. 
		\answerTODO{Yes}
		\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes.
		\answerTODO{Yes}
		\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. 
		\answerTODO{Yes}
		\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. 
		\answerTODO{Yes}
		\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. 
		\answerTODO{Yes}
	\end{enumerate}
	
	\item Does this paper include computational experiments? \answerTODO{Yes}
	\begin{enumerate}
		\item Any code required for pre-processing data is included in the appendix.
		\answerTODO{Yes}
		\item All source code required for conducting and analyzing the experiments is included in a code appendix.
		\answerTODO{Yes}
		\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes.
		\answerTODO{Yes}
		\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from.
		\answerTODO{Yes}
		\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. 
		\answerTODO{Yes}
		\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks.
		\answerTODO{Yes}
		\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics.
		\answerTODO{Yes}
		\item This paper states the number of algorithm runs used to compute each reported result.
		\answerTODO{Yes}
		\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. 
		\answerTODO{Yes}
		\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). 
		\answerTODO{Yes}
		\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. 
		\answerTODO{Yes}
		\item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. 
		\answerTODO{Yes}
		
	\end{enumerate}
	
\end{enumerate}
